Depth Extraction from Videos Using Geometric Context and Occlusion Boundaries

We present an algorithm to estimate depth in dynamic video scenes. We propose to learn and infer depth in videos from appearance, motion, occlusion boundaries, and geometric context of the scene. Using our method, depth can be estimated from unconstrained videos with no requirement of camera pose estimation, and with significant background/foreground motions. We start by decomposing a video into spatio-temporal regions. For each spatio-temporal region, we learn the relationship of depth to visual appearance, motion, and geometric classes. Then we infer the depth information of new scenes using piecewise planar parametrization estimated within a Markov random field (MRF) framework by combining appearance to depth learned mappings and occlusion boundary guided smoothness constraints. Subsequently, we perform temporal smoothing to obtain temporally consistent depth maps. To evaluate our depth estimation algorithm, we provide a novel dataset with ground truth depth for outdoor video scenes. We present a thorough evaluation of our algorithm on our new dataset and the publicly available Make3d static image dataset.

==> depthMRF.tex <==
%%\subsubsection{Data Term}
%%\label{sec:dataterm}
%%The term $g_i(.)$ in Equation 1 minimizes the total fractional depth error over all the pixels $k$ in a region $i$ in a frame. The fractional error is given as
%%\begin{equation}
%%\frac{\hat{d}_{k,i}-d_{k,i}}{d_{k,i}}=\hat{d}_{k,i} \cdot r_{k,i}^T\alpha_i-1
%%\end{equation}
%%Where $d$ is the ground truth depth and $\hat{d}$ is the predicted depth by the random forest mapping (Sec. \ref{sec:unary_depth}). The data term to minimize the total fractional error in a region $i$ with plane parameter $\alpha_i$ is given by:
%%\begin{equation}
%%g_i(\alpha_i|X_i,S_i)=\exp(\sum\limits_{k=1}^K||(r_{i,k}^T\alpha_i)\hat{d}_{i,k}-1||^2)
%%\end{equation}
%%
%%\subsubsection{Connectivity and Co-Planarity}
%%\label{sec:conn-cop}
%%We model the depth relation between a pair of regions by connectivity and co-planarity terms. Connectivity constrains the pixels on the boundary to be connected by minimizing the fractional distance between the pixels on the boundary $B_{ij}$ of regions $i$ and $j$ in absence of the occlusion boundary. The connectivity term is given as:
%%\begin{equation}
%%%\begin{split}
%%f_{\mbox{conn}}(\alpha_i,\alpha_j,y_{ij})=\exp(\frac{1}{|B_{ij}|}\sum\limits_{p\in B_{ij}}y_{ij}\\||(r_p^T\alpha_i-r_p^T\alpha_j)\sqrt{\hat{d_i}\hat{d_j}}||^2)
%%%\end{split}
%%\end{equation}
%%where $B_{ij}$ are the pixels on the boundary of regions $i$ and $j$ in a frame. The co-planarity term minimizes the fractional distance between the centres of the region and is given by:
%%\begin{equation}
%%%\begin{split}
%%f_{\mbox{cop}}(\alpha_i,\alpha_j,y_{ij})=\exp(y_{ij}||(r_q^T\alpha_i-r_q^T\alpha_j)\hat{d}_j||^2)
%%%\end{split}
%%\end{equation}
%%where $r_q$ is the center pixel of region $j$.
%%%\subsubsection{Inference}
%%%\label{sec:inference}
%%%To solve Equation 1 for $\alpha$ we find the MAP estimate by maximizing the $logP(\alpha|X,S,y)$. Then we can write Equation 1 as
%%%\begin{equation}
%%%\begin{split}
%%%{\alpha^\star}=\argmin_{\alpha}\sum\limits_{i=1}^N(\sum\limits_{k=1}^K||(r_{i,k}^T\alpha_i)\hat{d_{i,k}}-1||^2)+\\
%%%\sum\limits_{j\in N(i)}\frac{1}{|B_{ij}|}\sum\limits_{p\in B_{ij}} y_{ij}||(r_p^T\alpha_i-r_p^T\alpha_j)\sqrt{\hat{d_i}\hat{d_j}}||^2+\\
%%%\sum\limits_{j\in N(i)}\sum\limits_{q\in C_j}y_{ij}||(r_q^T\alpha_i-r_q^T\alpha_j)\hat{d_j}||^2\\
%%%\end{split}
%%%\end{equation} 
%%%where $N$ is the number of $2D$ regions in a video frame, $K_i$ is number of pixels in region $i$ in that frame, $C_j$ is the center of super-pixel $j$, $N(i)$ is the set of neighboring regions to the region $i$. We solve the above optimization problem using the L-BFGS algorithm \cite{liu1989limited} and compute the depth of each pixel $p$ in region $i$ using $d_{i,k}=1/r_{i,k}^T\alpha_i$. We compute depth for each 2D region in a frame using the MRF and then use a sliding window across frames to smooth out the inconsistencies in predicted depth.
%%


==> depthMRF_2.tex <==
\Paragraph{Depth Constraints}

Now, we solve the \Cref{eq:depth} using the L-BFGS algorithm \cite{liu1989limited} and compute the depth of each pixel $p$ in region $i$ using $d_{i,k}=1/r_{i,k}^T\alpha_i$. We compute depth for each 2D region in a frame using the MRF and then use a sliding window across frames to smooth out the inconsistencies in predicted depth.

==> ext_abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
\vspace{-0.3cm}
\noindent We present an algorithm to estimate depth in dynamic video scenes. We propose to learn and infer depth in videos from appearance, motion, occlusion boundaries, and geometric context of the scene. Using our method, depth can be estimated from unconstrained videos with no requirement of camera pose estimation, and with significant background/foreground motions. We start by decomposing a video into spatio-temporal regions. For each spatio-temporal region, we learn the relationship of depth to visual appearance, motion, and geometric classes. Then we infer the depth information of new scenes using piecewise planar parametrization estimated within a Markov random field (MRF) framework by combining appearance to depth learned mappings and occlusion boundary guided smoothness constraints. Subsequently, we perform temporal smoothing to obtain temporally consistent depth maps. We present a thorough evaluation of our algorithm on our new dataset and the publicly available Make3d static image dataset.
\end{abstract}
\vspace{-0.3cm}
\section{Introduction and Approach}
\label{sec:approach}
\vspace{-0.3cm}
Methods exploiting visual and contextual cues for depth can be used to provide an additional source of depth information to the structure from motion or multi-view stereo based depth estimation systems.
In this paper, we focus on texture features, geometric context, motion boundary based monocular cues along with co-planarity, connectivity and spatio-temporal consistency constraints to predict depth in videos. We assume that a scene can be decomposed into planes, each with its own planar parameters. We over-segment a video into spatio-temporal regions and compute depth cues from each region along with scene structure from geometric contexts. These depth cues are used to train and predict depth from features. However, such appearance to depth mappings are typically noisy and ambiguous. We incorporate the independent features to depth mapping of each spatio-temporal region within in a MRF framework that encodes constraints from scene layout properties of co-planarity, connectivity and occlusions. To model the connectivity and co-planarity in a scene, we explicitly learn occlusion boundaries in videos. To further remove the inconsistencies from temporal depth prediction, we apply a sliding window to smooth the depth prediction. Our approach doesn't require camera translation or large rigid scene for depth estimation. Moreover, it provides a source of depth information that is largely complementary to triangulation based depth estimation methods~\cite{saxena2007depth}.
%We learn occlusion boundaries using edgelet, color, geometric context, and flow-consistency features.
%In this paper, we propose an algorithm to estimate depth ordinary outdoor video scene.
\noindent\textbf{The primary contributions of our method to extract depth from videos are:}
\begin{list}{$\bullet$}
{\setlength{\leftmargin}{2ex}\setlength{\labelsep}{.5ex}\setlength{\parsep}{.4ex plus .2ex minus .1ex}\setlength{\itemsep}{0ex plus .1ex}\setlength{\topsep}{0ex plus .1ex}}
\item Adoption of a learning and inference approach that explicitly models appearance to geometry mappings and piecewise scene smoothness;
\item Learning and estimating occlusion boundaries in videos and utilizing these to constrain smoothness across the scene;
\item There is no requirement of a translating camera or a wide-baseline for depth estimation;
\item An algorithm for video depth estimation that is complementary to traditional structure from motion approaches, and that can incorporate these approaches to compute depth estimates for natural scenes;
%\item  We present a novel dataset providing ground truth depth for over 38 outdoor videos ($\sim$ 6400 frames). We also undertake a detailed analysis of contribution of monocular features in depth estimation and thorough evaluation on images and videos;
\end{list}
\vspace{-0.3cm}
\section{Experiments and Results}
\label{sec:result}
\vspace{-0.3cm}
%*** accuracy \\
\noindent We perform extensive experiments on video depth data to evaluate our algorithm. We perform 5-fold cross-validation over 36 videos ($\sim$ 6400 frames). We compute average log-error $|\log d - \log {\hat{d}}|$ and average relative error $|\frac{ d - \hat{d}}{d}|$ to report the accuracy of our method. We achieve an accuracy of $0.153$ log-error and $0.44$ on relative error (Table \ref{Table:result}). Figure \ref{fig:vid_depth_result} shows some example scenes from our dataset with ground truth and predicted depth.
Our approach for depth estimation can also be applied to images. We applied our algorithm over a publicly available Make3d depth image dataset \cite{saxena2009make3d}. Table \ref{table:make3d} gives the comparison of the single image variant of our approach with the state of the art and we achieve competitive results. It should be noted that our algorithm depends on occlusion boundary detection and geometric context (for which motion based features are important  and is not optimized to extract depth from single images.

%%% need to add legend for figures depth
\begin{figure}%[ht]
  \centering
      \includegraphics[width=0.45\textwidth]{vid_depth_examples_eccv_2.pdf}%{vidDepthResults_1.png}
      \vspace{-0.3cm}
  \caption{Examples of videos scenes, ground truth, and predicted depth by our method. Legend shows depth range from 0m (blue) to 80m (red). }
  \label{fig:vid_depth_result}
\vspace{-0.3cm}
\end{figure}

\begin{table}%[htb]

\begin{minipage}[t]{0.45\linewidth}
\centering
\small
\begin{tabular}{|c|c|c|c|}\hline
Features & $log10$  & rel-depth \\\hline
ALL & 0.153  & 0.44\\\hline
App.+Flow & 0.176  & 0.533\\\hline
Appearance & 0.175  & 0.512\\\hline
%%%% need to compute the numbers below, Just for completion using random numbers
%\emph{mix} & 0.5   \\\hline
\end{tabular}
%\vspace{-03.cm}
\caption{Performance of our algorithm on video dataset, combining appearance, flow, and surface layout features give best accuracy.}
\label{Table:result}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}[t]{0.5\linewidth}
\centering
\small
\begin{tabular}{|c|c|c|c|}\hline
Algorithm & $log10$  & rel-$log$ \\\hline
SCN \cite{saxena2005learning} & 0.198  & 0.530\\\hline
HEH \cite{HoiemIJCV2007} & 0.320  & 1.423\\\hline
Baseline \cite{saxena2009make3d} & 0.334  & 0.516\\
PP-MRF \cite{saxena2009make3d} & 0.187  & 0.370\\
Depth Transfer \cite{karsch2012depth} & 0.148 & 0.362  \\\hline
Sematic Labels \cite{liu2010single}  & 0.148 & 0.379 \\\hline
\textbf{*Geom. Context}  & & \\
\textbf{Occl. Bound.} & \textbf{0.159} & \textbf{0.386} \\\hline
%\emph{mix} & 0.5   \\\hline
\end{tabular}
%\vspace{-0.3cm}
\caption{Our approach can also be applied to images. We apply it to Make3d depth image dataset \cite{saxena2009make3d}.}
%\caption{Comparison on make3d dataset. best results in other publications are 0.148 and 0.370, respectively. I will try to improve it next week.}
\label{table:make3d}
\end{minipage}
\vspace{-0.5cm}
\end{table}


==> intro-Harpreet.tex <==
\section{Introduction}
\label{sec:intro}

\noindent Human vision is capable of infering the 3D structure of a scene even when observed in monocular imagery. However, estimating 3D structure from videos of general scenes still remains a challenging problem in computer vision. 
A large majority of prior work on 3D structure extraction from a monocular camera, like structure from motion and multi-view stereo relies on pose estimation and  triangulation to estimate depth maps \cite{zhang2009consistent,newcombe2010live}. However, most of these geometric methods for depth estimation require camera translation, absence of large independently moving foreground objects, and rigid textured image regions that can be matched across views. These assumptions are not true in many consumer videos, which tend to have people moving around in the foreground,  small translations and potentially non-rigid background (see Figure \ref{fig:intro}).

%Automatic 3D structure estimation algorithms will have significant impact on applications in visual surveillance, visual metrology, autonomous navigation and augmented reality systems. 
    

\begin{figure}[t!]
  \centering
      \includegraphics[width=0.4\textwidth]{depth_intro_1.pdf}%{intro_depth.png}
  \caption{A video scene (left) and the depth map (right) }
  \label{fig:intro}
\end{figure}

In this paper, instead of using triangulation based constraints,  we pose the problem of depth estimation in terms of statistical learning and inference. Rather than explicitly triangulating points from the video, we propose to learn a mapping of monocular cues to depth. There are numerous monocular cues such as texture variations, occlusion boundaries,  defocus, color/haze, surface layout, and size/shape of known objects, that contain useful and important cues for depth information. 

Specifically we focus on texture features, geometric context, motion boundary based monoculor cues along with co-planarity, connectivity and spatio-temporal consistency constraints to predict depth in videos. We assume that a scene can be decomposed into planes each with its own planar parameters. We over-segment a video into spatio-temporal regions and compute depth cues from each region along with scene structure from geometric contexts. These depth cues are used to train and predict depth from features. However, such appearance to depth mappings are typically noisy and ambiguous. We incorporate the independent features to depth mapping of each spatio-temporal region within in an MRF framework that encodes constraints from $3D$ scene properties of co-planarity, connectivity and occlusions. To model the connectivity and co-planarity in a scene, we explicitly learn occlusion boundaries in videos. To further remove the inconsistencies from temporal depth prediction, we apply a sliding window to smooth the depth prediction. Our approach doesn't require camera translation or large rigid scene for depth estimation. Moreover, it provides a source of depth information that is largely complementary to triangulation based depth estimation methods~\cite{saxena2007depth}.

%We learn occlusion boundaries using edgelet, color, geometric context, and flow-consistency features.
%In this paper, we propose an algorithm to estimate depth ordinary outdoor video scene. 

\noindent\textbf{The primary technical contributions of our method to extract depth from videos are:}
\begin{list}{$\bullet$}
{\setlength{\leftmargin}{2ex}\setlength{\labelsep}{.5ex}\setlength{\parsep}{.4ex plus .2ex minus .1ex}\setlength{\itemsep}{0ex plus .1ex}\setlength{\topsep}{0ex plus .1ex}}
\item Adoption of a learning and inference approach that explicitly models appearance to geometry mappings and piecewise scene smoothness; 
\item Learning and estimating occlusion boundaries in videos and utilizing these to constrain smoothness across the scene; 
\item An algorithm for video depth estimation that is complementary to traditional structure from motion approaches, and that can incorporate these approaches to compute depth estimates for natural scenes of a much wider variety then what the SFM approache can handle; 
\item A new co-registered video and depth dataset with over $38$ outdoor videos ($\sim$ $6400$ frames) and pixel registered depth maps. 
\end{list}

We also undertake a detailed analysis of contribution of monocular features in depth estimation and evaluation on images and videos. 

 




